Corruption-Robust Lipschitz Contextual Search

I study the problem of learning a Lipschitz function with corrupted binary signals. The learner tries to learn a $L$-Lipschitz function $f: [0,1]^d \rightarrow [0, L]$ that the adversary chooses. There is a total of $T$ rounds. In each round $t$, the adversary selects a context vector $x_t$ in the input space, and the learner makes a guess to the true function value $f(x_t)$ and receives a binary signal indicating whether the guess is high or low. In a total of $C$ rounds, the signal may be corrupted, though the value of $C$ is \emph{unknown} to the learner. The learner's goal is to incur a small cumulative loss. This work introduces the new algorithmic technique \emph{agnostic checking} as well as new analysis techniques. I design algorithms which: for the symmetric loss, the learner achieves regret $L\cdot O(C\log T)$ with $d = 1$ and $L\cdot O_d(C\log T + T^{(d-1)/d})$ with $d > 1$; for the pricing loss, the learner achieves regret $L\cdot \widetilde{O} (T^{d/(d+1)} + C\cdot T^{1/(d+1)})$.

==> old/oldanalysis.tex <==
\subsection{Analysis for Weight Update}
\section{Algorithm for the Absolute Loss}
\begin{algorithm}
\begin{algorithmic}
\caption{Learning with Weight Update}
\State Maintain a partition of intervals of the input space throughout learning process
\State Partition initialized as $\ceil{8L}$ intervals with length less than $1/8L$ each
\For {round $t = 1, 2, \dots, T$}
    \State Receive context $x_t$
    \State Find interval $I_t$ such that $x_t \in I_t$
    \If {The concentration endpoint of $I_t$ not queries}
        \State Query concentration endpoint of $I_t$ 
        \State If anomaly detected, mark $I_t$ as untruthful. 
        \State Else, mark the concentration region of $I_t$. 
    \EndIf
    \If {$I_t$ queried less than $c_0$ times}
        \State Find midpoint $q$ in concentration region, specifically find point $q$ such that $f([q + L\cdot\len(I_t), >]; I_t) = f([<, q - L\cdot\len(I_t)]; I_t)$
        % \State Find midpoint $q$ in $[0,1]$
    \Else \Comment{This interval is dishonest}
        \State Find midpoint $q$ in $[0,1]$
    \EndIf
    \State Submit guess $q$, receive binary feedback $\sigma_t$
    \If {$\sigma_t = 1$} \Comment{If guess is high}
        \State update $f[>q + \len] = 0.5 \cdot f[>q + \len] $
        \State update $f[<q + \len] = 1.5 \cdot f[<q + \len] $
        \State Normalize
    \Else \Comment{If guess is low}
        \State update $f[>q - \len] = 1.5 \cdot f[>q - \len] $
        \State update $f[<q - \len] = 0.5 \cdot f[<q - \len] $
        \State Normalize
    \EndIf

    \If{$f(I_t) < 0.1$}
    \State Split and reset weight
    \EndIf
\EndFor
\State \dots
\end{algorithmic}
\end{algorithm}

Some definitions are first provided that will aid the analysis. 

\begin{definition}[Corrupted Interval]
    An interval is called a corrupted interval if any round inside the interval is corrupted. 
\end{definition}

\begin{definition}[Correcting Interval]
    An interval is called a correcting interval if any round inside the interval is uncorrupted and the parent interval is corrupted. 
\end{definition}

\begin{definition}[Truthful Interval]
    An interval is called a truthful interval if any round inside the interval is uncorrupted and the parent interval is either a correction interval or a truthful interval. 
\end{definition}

\begin{definition}[Consistent Region]
    The consistent region of an interval $I$ is defined as $[M - L\cdot \len, m + L\cdot \len]$, where $m = \dots, M = \dots$
\end{definition}

\begin{definition}[Concentrated region]
    Consider an interval $I$. If there exists an interval $[a, b]$ such that $f([a,b]; I) > u$ we say the interval $I$ is concentrated with level $u$ at $[a,b]$. 
\end{definition}

\begin{claim}
For an interval $I$, it is concentrated with level $0.8$ at some interval with length $2\cdot \len$ right before splitting. Equivalently, for any interval $I'$, it is concentrated with level $0.8$ at some interval with length $4\cdot \len$ at the beginning. 
\end{claim}

\begin{lemma}
A correction interval at depth $h$ takes at most $O(c_0 + h)$ rounds before splitting. Further, the correction interval will be concentrated around the consistent region right before splitting. 
\end{lemma}
\begin{proof}
    Let $I$ be a correction interval. Consider the consistent region of interval $I$. 
    At the start the consistent region will have volume $2^{-h}$. 
    Suppose for sake of contradiction $I$ is not splitted after $c_0$ queries. Then for every query in $I$, we must have $p > 0.1$, and hence the volume of the consistent region gets multiplied by a constant factor. After $O(h)$ rounds we will have the volume of the consistent region greater than 1, contradiction. 

    \szcomment{TODO concentrated around consistent region? }
\end{proof}

\begin{lemma}
    At the beginning of a truthful interval, the interval is focused on the consistent region. 
\end{lemma}
\begin{proof}
    If the parent interval is truthful, then yes. If the parent interval is correction interval? \szcomment{TODO}\dots
\end{proof}

\begin{lemma}
    A truthful interval at depth $h$ takes at most $O(c_0)$ queries before splitting, and each query accumulates loss at most $O(2^{-h})$. 
\end{lemma}
\begin{proof}
Consider the consistent region. Suppose the interval has received $c_0$ queries. Then for each query, the consistent region is getting its volume multiplied by some constant. After $c_0$ rounds, its volume will be greater than 1. Hence the interval splits in at most $c_0$ queries. \szcomment{TODO Each query accumulates loss $2^{-h}$. }
\end{proof}

\begin{lemma}
    Consider a corrupted interval and let there be $c_1$ rounds corrupted, then the corrupted interval splits in at most $O(c_1)$ queries. 
\end{lemma}
\begin{proof}
    
\end{proof}

\begin{theorem}
Total loss bounded by $O(C\log T)$. 
\end{theorem}


==> sections/TODO.tex <==
Better names
Sincere interval
abiding interval
Safe

Bisecting needs to stop at level log T
Either stop bisecting
Or don't require Yj to be that small

Sparse Contextual Search

==> sections/algorithmsWithAlgX.tex <==
\begin{algorithm}[h]
\caption{Learning with corrupted binary signals under symmetric loss for $d=1$}
\label{algo:1dabsolute}
\begin{algorithmic}[1]
\State Learner maintains a partition of intervals $I_j$ of the input space throughout learning process
\State For each interval $I_j$ in the partition, learner stores a sanity check interval $S_j$, and maintains an associated range $Y_j$
\State The partition is initialized as $8$ intervals $I_j$ with length $1/8$ each, and each $I_j$ has associated range $Y_j$ and sanity check interval $S_j$ set to $[0,L]$
\For {round $t = 1, 2, ..., T$}
    \State Learner receives context $x_t$
    \State Learner finds interval $I_j$ such that $x_t \in I_j$
    \State Let $Y_j$ be the associated range of $I_j$
    \If {Exists an endpoint of $S_j$ not yet queried} %\label{algo:queryendpt_beg}
        \State Learner selects an unqueried endpoint of $S_j$ as guess
        \If {Learner guessed $\min(S_j)$ and $\sigma_t = 1$, or guessed $\max(S_j)$ and $\sigma_t = 0$} 
        \State Mark $I_j$ as unsafe \Comment{Contamination found in the current interval}
        \EndIf
        \If {Both endpoints of sanity check interval $S_j$ have been queried}
            \If {$I_j$ marked unsafe}
                \State Set range $Y_j := [0,L]$ \label{algoline:marked_rangeset}
            \Else
                \State Set range $Y_j = [\min(S_j) - L\cdot \len(I_j)), \max(S_j) + L\cdot \len(I_j))] \cap [0,L]$ \label{algoline:unmarked_rangeset}
            \EndIf
        \EndIf %\label{algo:queryendpt_end}
    \Else %{$I_t$ not marked unsafe} \label{algo:notmarked_beg}
        \State $Y_j := \algmq(I_j, Y_j)$
        \If { $\len(Y_j) < \max( 4 L\cdot \len(I_j), 4 L / T )$ }  \LineComment{Check if associated range $Y_j$ has shrunk enough}
            \State Bisect $I_j$ into $I_{j1}, I_{j2}$, set $S_{j1} = Y_j, S_{j2} = Y_j$ 
        \EndIf %\label{algo:notmarked_end}
    %\Else \Comment{$I_t$ is marked dishonest} \label{algo:dishonest_begin}
        %\State Start from scratch until converge, takes $\log T$ steps \label{algo:test}
        
        %\State Let $\set{[], [], []}$ be the sequence of feasible region (endpoints? ) on the path to $I_t$. 
        %\State Perform binary search on this path and find the first interval [] that contains $f(I_t)$. \Comment{Takes $\log\log T$ steps}, set feasible region $I_t = []$
        %\State From this point perform binary search and shrink feasible region \Comment{Takes $c$ steps, where $c$ is number of corruptions before reaching a correction interval? }
    \EndIf 
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm2e}
\caption{Midpoint query procedure: $\algmq(I_j, Y_j)$}
\label{algo:midpt_query}
    \State Input: $I_j, Y_j$
    \State Let $q$ be midpoint of $Y_j$
    \State Learner queries $q$
    \If {$\sigma_t$ = 1}
        % \State Set $Y'_j := [\min(Y_j), q_t + L\cdot\len(I_j)]$
        \State Set $Y'_j := [0, q_t + L\cdot\len(I_j)] \cap Y_j$
        \szcomment{This and above should be equivalent}
    \Else
        % \State Set $Y'_j := [q_t - L\cdot\len(I_j), \max(Y_j)]$
        \State Set $Y'_j := [q_t - L\cdot\len(I_j), 1] \cap Y_j$
        \szcomment{This and above should be equivalent}
    \EndIf
    \State Return $Y'_j$
\end{algorithm2e}


\begin{algorithm}[h]
\caption{Learning with corrupted binary signal under pricing loss with uniform discretization}
\label{algo:pricing}
\begin{algorithmic}[1]
\State Set parameter $\eta_0 = T^{-1/(d+1)}$, sanity check schedule $\tau_0$
\State Learner uniformly discretizes input space into hypercubes with lengths no larger than $\eta_0$ each
\State For each hypercube $I_j$, learner maintains an associated range $Y_j$ (initialized as $[0, L]$), query count $c_j$ (initialized as $0$)
% \State Set $\eta = 10 L \cdot T^{1/(d+1)}$
\For {$t = 1, 2, ..., T$}
    \State Learner receives context $x_t$
    \State Learner finds hypercube $I_j$ such that $x_t \in I_j$
    \State Let $Y_j$ be the associated range of $I_j$
    \If {$\len (Y_j) < 10 L \cdot \eta$} \Comment{The interval is pricing-ready}
        \State $c_j := c_j + 1$
        \If { $c_j > \tau_0$ } 
            \State Query $\max(Y_j)$
            \State Set $c_j := 0$
        \Else 
            \State Query $\min(Y_j)$
        \EndIf
        \If {Learner is surprised} \LineComment{Learner is surprised if queried $\max(Y_j)$ and $\sigma_t = 0$, or queried $\min(Y_j)$ and $\sigma_t = 1$}
            \State Set $Y_j := [0,L]$ \Comment{Reset the range of $Y_j$}
            \State Set $c_j := 0$
        \EndIf
    % \ElsIf {Exists an endpoint in $S_j$ not queried} %\label{algo:queryendpt_beg}
    %     \State Query an unqueried endpoint of $S_j$
    %     \If {Queried $\min(S_j)$ and $\sigma_t = 1$, or queried $\max(S_j)$ and $\sigma_t = 0$} 
    %     \State Mark $I_j$ as unsafe \Comment{Contamination found in the current interval}
    %     \EndIf
    %     \If {Both endpoints of $S_j$ have been queried}
    %         \If {$I_j$ marked unsafe}
    %             \State Set range $Y_j := [0,1]$ \label{algoline:marked_rangeset}
    %         \Else
    %             \State Set range $Y_j = [\min(S_j) - L\cdot \len(I_j)), \max(S_j) + L\cdot \len(I_j))] \cap [0,1]$ \label{algoline:unmarked_rangeset}
    %         \EndIf
    %     \EndIf %\label{algo:queryendpt_end}
    \Else %{$I_t$ not marked unsafe} \label{algo:notmarked_beg}
        \State $Y_j := \algmq(I_j, Y_j)$
        % \If { $\len(Y_j) < 4 L\cdot \len(I_j)$}  \Comment{associated range $Y_j$ has shrunk enough}
        %     \State Bisect each side of $I_j$ to form $2^d$ new hypercubes, each with length $...$
        % \EndIf %\label{algo:notmarked_end}
    \EndIf
    %\Else \Comment{$I_t$ is marked dishonest} \label{algo:dishonest_begin}
        %\State Start from scratch until converge, takes $\log T$ steps \label{algo:test}
        
        %\State Let $\set{[], [], []}$ be the sequence of feasible region (endpoints? ) on the path to $I_t$. 
        %\State Perform binary search on this path and find the first interval [] that contains $f(I_t)$. \Comment{Takes $\log\log T$ steps}, set feasible region $I_t = []$
        %\State From this point perform binary search and shrink feasible region \Comment{Takes $c$ steps, where $c$ is number of corruptions before reaching a correction interval? }
    %\EndIf %\label{algo:dishonest_end}
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Learning with corrupted binary signal under symmetric loss with $d > 1$}
\label{algo:highDsymm}
\begin{algorithmic}[1]
\State Learner maintains a partition of hypercubes $I_j$ of the input space $[0,1]^d$ throughout learning process
\State For each hypercube $I_j$, learner stores a sanity check interval $S_j$ and maintains an associated range $Y_j$
\State The partition is initialized as a single hypercube with sanity check interval $S_j$ set to $[0, 8L]$
\For {round $t = 1, 2, ..., T$}
    \State Learner receives context $x_t$
    \State Learner finds hypercube $I_j$ such that $x_t \in I_j$
    \State Let $Y_j$ be the feasible interval of $I_j$
    \If {Exists an endpoint of $S_j$ not queried} %\label{algo:queryendpt_beg}
        \State Query an unqueried endpoint of $S_j$
        \If {Queried $\min(S_j)$ and $\sigma_t = 1$, or queried $\max(S_j)$ and $\sigma_t = 0$} 
        \State Mark $I_j$ as unsafe \Comment{Contamination found in the current interval}
        \EndIf
        \If {Both endpoints of $S_j$ have been queried}
            \If {$I_j$ marked unsafe}
                \State Set range $Y_j := [0, 8L]$ \label{algoline:highd_marked_rangeset}
            \Else
                \State Set range $Y_j = [\min(S_j) - L\cdot \len(I_j)), \max(S_j) + L\cdot \len(I_j))] \cap [0,1]$ \label{algoline:highd_unmarked_rangeset}
            \EndIf
        \EndIf %\label{algo:queryendpt_end}
    \Else %{$I_t$ not marked unsafe} \label{algo:notmarked_beg}
        \State $Y_j := \algmq(I_j, Y_j)$
        \If { $\len(Y_j) < \max (4 L\cdot \len(I_j), 4L / T )$ }  \Comment{associated range $Y_j$ has shrunk enough}
            \State Bisect each side of $I_j$ to form $2^d$ new hypercubes each with length $\len(I_j) / 2$
            \State For each new hypercube $I_{ji}$ ($1\le i \le 2^d$) set $S_{ji} = Y_j$
        \EndIf %\label{algo:notmarked_end}
    %\Else \Comment{$I_t$ is marked dishonest} \label{algo:dishonest_begin}
        %\State Start from scratch until converge, takes $\log T$ steps \label{algo:test}
        
        %\State Let $\set{[], [], []}$ be the sequence of feasible region (endpoints? ) on the path to $I_t$. 
        %\State Perform binary search on this path and find the first interval [] that contains $f(I_t)$. \Comment{Takes $\log\log T$ steps}, set feasible region $I_t = []$
        %\State From this point perform binary search and shrink feasible region \Comment{Takes $c$ steps, where $c$ is number of corruptions before reaching a correction interval? }
    \EndIf %\label{algo:dishonest_end}
\EndFor
\end{algorithmic}
\end{algorithm}

==> sections/app_Leffect.tex <==
\section{Effect of $L$}
This sections gives a brief description on how $L$ affects the loss guarantees. If $L < 1$, then the function is assumed to take the range $[0, L]$. 

If $L > 1$, then the function is assumed to take the range $[0,1]$. 

\szcomment{Other option is to assume function take range $[0, L]$. }

==> sections/app_covering.tex <==
\section{Covering Dimension Based}

\begin{algorithm}[htbp]
\caption{Covering Dimension Based}
\label{algo:covering}
\begin{algorithmic}
\State Learner start with uniform density over $\cF(1/T^2)$, the $1/T^2$ covering of $\cF$
\For{$t = 1, 2, ..., T$}
    \State Learner finds $m_t$ such that $\Pr[f(x_t) \ge m_t] \ge 1/2$, $\Pr[f(x_t) \le m_t] \ge 1/2$
    \State Learner guesses $q_t$ uniformly chosen from $[m_t - 1/T, m_t + 1/T]$
    \State $w(f) = w(f) * (1 + c)$ if $\sigma(q_t - f(x_t)) = \sigma_t$
    \State $w(f) = w(f) * (1 - c)$ if $\sigma(q_t - f(x_t)) = 1-\sigma_t$
    \State Normalize
\EndFor
\end{algorithmic}
\end{algorithm}

%In addition, $f(x_t) = q_t$ happens with $0$ probability for any $f\in \cF(1/T^2)$. 
\begin{lemma}
    With probability $1 - \frac{1}{2T}$, $f^*(x_t)$ and $f_0(x_t)$ are on the same side of $q_t$.
\end{lemma}
\begin{proof}
    Fix any $x_t, m_t$. Note that $\abs{f_0(x_t) - f^*(x_t)} < \frac{1}{T^2}$. With probability $1 - \frac{1}{2T}$, $f_0(x_t)$ and $f^*(x_t)$ will be on the same side of a randomly drawn point in the interval $[m_t - 1/T, m_t + 1/T]$. 
\end{proof}

In accordance with the possibly corrupted signal $\sigma_t$, let $W_t^-$ be the total density of $f(x_t)$ not on the same side of $q_t$, and let $W_t^+$ be the total density of $f(x_t)$ on the same side of $q_t$. 
\begin{align*}
    W_t^- &= w ( \set{ f: \sigma( q_t - f(x_t)) = \sigma_t} ) \\
    W_t^+ &= w ( \set{ f: \sigma( q_t - f(x_t)) = 1 - \sigma_t} ) 
\end{align*}
Further define $\Delta^+ = W_t^+ - 1/2$, then $\Delta^+ \in [-1/2, 1/2]$. Intuitively, the algorithm makes more progress when $\Delta^+$ is closer to 0. 

Assume the signal was uncorrupted at round $t$, then for any $f(x_t)$ on the same side as $q_t$, the density update follows 
\begin{align*}
w(f) &= w(f) \cdot (1 + c) / [(1+c) W^+ + (1-c) W^-] \\
&= w(f) \cdot (1 + c) / (1 + 2c\Delta^+)
\end{align*}
If $f(x_t)$ is on different side as $q_t$,
\begin{align*}
w(f) &= w(f) \cdot (1 - c) / [(1+c) W^+ + (1-c) W^-] \\
&= w(f) \cdot (1 - c) / (1 + 2c\Delta^+). 
\end{align*}

\begin{lemma}
If the signal is uncorrupted and $\abs{f^*(x_t) - m_t} > 2/T$, then weight of $f_0$ grows. 
\end{lemma}
\begin{proof}
Recall $m_t$ is the median, and $q_t$ is the perturbed version. If $f^*$ and $m_t$ are at least $2/T$ apart, then $f^*$ and $f_0$ will be on same side of $q_t$. With probability $1/2$, the learner has $W^- \ge 1/2$, and consequently $w_{t+1}(f_0) \ge w_t(f_0) \cdot (1 + c)$. With the remaining probability $w_{t+1}(f_0) \ge w_t(f_0)$. 

Hence the learner has the following:
\begin{align*}
    \Ex[w_{t+1}(f_0)] \ge \frac{2+c}{2} w_t(f_0)
\end{align*}
\begin{align*}
    \Ex \left[ \frac{1} {w_{t+1}(f_0)} \right] \le \frac{2+c}{2 + 2c} \cdot \frac{1}{w_t(f_0)}
\end{align*}
\end{proof}

\begin{lemma}
    If the signal is corrupted, then
    \begin{align*}
        w_{t+1}(f_0) \ge w_t(f_0)\cdot (1 - c) / (1 + c)
    \end{align*}
    \begin{align*}
        \frac{1}{w_{t+1}(f_0)} \le \frac{1+c}{1-c} \cdot \frac{1}{w_t(f_0)}
    \end{align*}
\end{lemma}
\begin{proof}
Follows from update rule. 
\end{proof}

\begin{lemma}
If the signal is uncorrupted, then
\begin{align*}
    ...
\end{align*}
\end{lemma}
\begin{proof}
    With $1 - \nicefrac{1}{2T}$ probability, $f^*$ and $f_0$ are on same side of $q_t$ and $w_{t+1}(f_0) \ge w_t(f_0)$. Otherwise with the remaining $\nicefrac{1}{2T}$ probability, 
    \begin{align*}
        w_{t+1}(f_0) \ge w_t(f)\cdot \frac{1-c}{1+c}
    \end{align*}
    Hence
    \begin{align*}
        \Ex[w_{t+1}(f_0)] &\ge (1 - \frac{1}{2T}) w_t(f) + \frac{1}{2T} \cdot \frac{1-c}{1+c} \cdot w_t(f) \\
        &\ge w_t(f) [ 1 - \frac{1}{2T}\cdot \frac{2c}{1 + c} ]
    \end{align*}
    \begin{align*}
        \Ex[\frac{1}{w_{t+1}(f_0)}] &\le (1 - \frac{1}{2T}) \cdot \frac{1}{w_t(f)} + \frac{1}{2T} \cdot \frac{1+c}{1-c} \cdot \frac{1}{w_t(f)} \\
        &\le \frac{1}{w_t(f)} \left( 1 + \frac{1}{2T}\cdot \frac{2c}{1 - c} \right)
    \end{align*}
\end{proof}

\begin{theorem}
The main theorem ...
\end{theorem}
\begin{proof}
    Define the variables:
    $s_1 = 1/\abs{N}$. 
    \begin{align*}
        s_t &= \frac{1+c}{1-c} \text{ if } \text{corrupted} \\
        s_t &= \frac{2+c}{2 + 2c} \cdot s_{t-1}\text{ if } \abs{} > 2/T, \text{uncorrupted} \\
        s_t &= 1 + \frac{1}{2T}\cdot\frac{2c}{1-c} \text{if } \abs{} < 2/T, \text{uncorrupted}
    \end{align*}

    Define the stochastic process
    \[
    Y_t = \frac{1}{s_t\cdot w_t(f_0)}
    \]
    Then $\Ex[Y_{t+1}] \le Y_{t}$. 

    Let $C$ be the total number of corrupted rounds, let $C'$ be the total number of uncorrupted rounds with $\abs{...} < 2/T$. Then $s_T$ can be upper bounded: 
    \begin{align*}
        s_T \le \frac{1}{N} \cdot  (\frac{1+c}{1-c})^{C} \cdot (\frac{2+c}{2+2c})^{C'} \cdot (1 + \frac{1}{2T})^T \le O(1/T)
    \end{align*}

    Hence
    \[
    Y_T = \frac{1}{s_T w_T} \ge \frac{1}{s_T} \ge \Omega(T)
    \]
\end{proof}

\szcomment{TODO remove log T factor??}
\subsection{Removing the $\log T$ factor}
Try using a multi-scale argument. 
Show when guess is $\epsilon$-far, then all $\epsilon$-close hypothesis gets multiplied by a constant factor. This is because any $\epsilon$-close hypothesis must be on the same side of the true hypothesis $f^*$. 

Existing results. 
\begin{enumerate}
    \item $O(d^2)$ loss using multiscale discretization. Deterministic signals, no corruption. No density. Select the midpoint from suitable layer. Then keep all hypothesis in layer $i$ that is $z_i$-consistent to make sure true hypothesis never eliminated. 
    \item $O(d\log T)$ loss using single scale discretization. Noisy signals. Use density. Compute the midpoint. Then the weight of $f_0$ multiplied by constant factor whenever guess is $2/T$ far. Also need to make sure when guess is $2/T$ close, the weight of $f_0$ does not decrease too much, to achieve this add perturbation to guess so that they are on same side. 
\end{enumerate}

To recap, the argument for $\log T$ version with density update goes as follows. When guess $2/T$-far, then $f_0$ must be on same side as $f$, and will get multiplied by constant factor. This can happen at most $O(d\log T)$ times. 

The argument for regret constant in $T$ uses a multiscale argument. 

Let $N_z(\cF)$ be any $z$-covering of the hypothesis class $\cF$. Define the $\gamma$-window median to be the point $q$ such that
\[
w( > q + \gamma) > 1/4, w( < q - \gamma) > 1/4
\]
If there is no such $q$, then the density does not have a $\gamma$-window median. 

The learner keeps a density $w_t$ for each layer of discretization $F^{z_i}$, here $z_i = 3^-d$ so that layer $i$ provides a $z_i$-covering. The density $w^i_1$ is initialized as the uniform density. 

Ideally the algorithm should satisfy the following:
\begin{enumerate}
    \item If the guess was $2z_i$-far, then $f_i \ge f_i \cdot \frac{1.5}{1.25}$. 
    \item If uncorrupted, the weight does not decrese. 
    \item If corrupted, weight decrease by at most $1/3$. 
\end{enumerate}

The analysis focuses on the density of $f_1, f_2, ...$, the density of $z_i$-close approximations. 

The algorithm is summarized as follows. 

\begin{algorithm}
\caption{Covering Dimension based}

\begin{algorithmic}[1]

\State Learner maintains density for all layers

\For {$t = 1, 2, ..., T$} 
    \State Find the smallest index $i$ such that there exists a $z_i$-window median, let the median be $q$. 
    \State Learner queries $q$ and receives possibly corrupted signal $\sigma_t$
    \For {$i = 1, 2, \dots$} 
        \State Update the density of all $f$ in layer $i$ as follows: 
        \begin{align*}
            w(f) &= w(f) * 1.5 \text{ if } f(x) > q - z_i \\
            w(f) &= w(f) * 0.5 \text{ otherwise }
        \end{align*}
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

Let $f_i$ be the function in layer $i$ such that 
\[
\norm{f_i - f^*}_\infty < z_i
\]

\begin{lemma}
    Fix a round $t$. Assume the guess was $2z_i$-far. Then $f_{i}$ is multiplied by a constant factor for any $i$. 
\end{lemma}
\begin{proof}
    We show that there exists a point $q$ such that $q$ is the $\gamma$-window median for any $\gamma \le z_i$. 
\end{proof}



==> sections/app_lower.tex <==
\subsection{Lower Bound}
\szcomment{Comment: Different approach to state the upper bound. }

It is natural to wonder whether the dependence on $C$ in the above theorem is tight. That is, whether one can achieve a bound of the form:
\[
\widetilde{O}(T^{d/(d+1)} + C)
\]

The below lower bound shows this is not possible. 

\begin{theorem}
Assume $L = 1$. Let $A$ be any algorithm to which the corruption budget $C$ is unknown. Suppose $A$ achieves a cumulative pricing loss $R(T) = o(T)$ when $C = 0$. Then, there exists some $C = 4R(T)$, such that the algorithm suffers $\Omega(T)$ regret. 
\end{theorem}

\begin{proof}
Let us consider two environments. In the first environment, the adversary chooses $f(x)=0.5$. In the second environment, the adversary chooses $f(x)=1$. 
	
The adversary adopts the following strategy. In the first environment where $f(x) = 0.5$, the adversary never corrupts the signal. In the second environment where $f(x) = 1$, the adversary corrupts the signal whenever the seller queries a point above $0.5$. Hence, the adversary manipulates the seller into thinking the true price is 0.5. 

Now we know the algorithm achieves regret $R(T)$ when $C=0$. Then, when $f(x) = 0.5$, the seller can only query values above $0.5$ for at most $2R(T)$ times. However, by choosing $C = 2R(T)$, the adversary can make the two environments indistinguishable to the seller. Hence the seller necessarily incurs $\Omega(T)$ regret. 
\end{proof}

The next theorem shows a lower bound when the corruption budget $C$ is known. We will prove our lower bound against a randomized adversary. Define an instance as the tuple $(f, C, \cS)$, where $f$ is the Lipschitz function, $C$ is the corruption budget, and $\cS$ is the corruption strategy of the adversary. The randomized adversary draws a problem instance from some probability distribution $\cD$, and the corruption budget is defined as the expected value of $C$ under distribution $\cD$. 
\begin{theorem}
Let $0 < C < T$ be the corruption budget and is known to the learner. Then for any algorithm, there exists some corruption strategy such that the learner incurs $\Omega(\sqrt{CT})$ regret. 
\end{theorem}
\begin{proof}
Consider the following corruption strategy. The space is discretized into $\sqrt{T/C}$ hypercubes of equal length. The context that the adversary selects will be the center of each hypercube, and the value at each context will be 0.5 except for one context which has value $0.5 + \eps$. Each hypercube will be selected by the adversary for $\sqrt{CT}$ rounds. The adversary will corrupt the first $C$ queries in the hypercube which has value $0.5+\eps$. At a high level, the learner can only detect the hypercube with value $0.5 + \eps$ if he performs checking rounds in every hypercube for at least $C$ rounds. Alternatively, if the learner does not perform checking query, he will incur regret $\eps \sqrt{CT}$. 

Can we choose there to be $1/\eps = \sqrt{T/C}^{1/d}$ hypercubes that has value $0.5+\eps$? 
\end{proof}

Difficulty should be the learner does not know how many times a interval will be queried. 

==> sections/covering.tex <==
\section{Covering Dimension Based Bounds}
This sections gives a corrupted robust algorithm for learning general hypothesis classes with finite covering dimension. The problem setup remains the same with the Lipschitz function class being replaced by a general hypothesis class. It is shown here that the density update algorithm in~\cite{liu2021optimal} achieves loss $O(Cd\log T)$. 

Let $\cF$ be a hypothesis class and $\cX$ be the input space. For any function $f\in\cF$, $f$ maps elements in $\cX$ to $\cR$. An adversary selects a ground truth hypothesis $f^*$. At each round, the adversary selects an input $x_t$, and the learner submits a guess $q_t$ upon observing the input. The adversary then gives the learner a binary feedback $\sigma_t$, and the learner suffers the symmetric loss $\ell_t = \abs{f^*(x_t) - q_t}$. 

The algorithm works as follows. The learner takes a $\frac{1}{T^2}$-covering of the hypothesis space $\cF$.  Denote the covering set by $C_\cF$, then there exists a element $f_0$ in the covering set such that $\norm{f_0 - f^*}_\infty < 1/T^2$. 

At initialization, the learner sets a uniform density in the covering set. Subsequently in each round, the learner finds the number $m_t$ such that $y_t$ is the median and queries $q_t$, a perturbed version of $m_t$. 

The analysis focuses on the density of $f_0$. Assume in some round, the query point is far from $f^*(x_t)$ with a distance at least $2/T$ and that the signal was uncorrupted, then density of $f_0$ will be multiplied by a constant. For any corrupted rounds, the density of $f_0$ is shrinks by at most a constant factor. 

\begin{theorem}
    Main theorem. 
\end{theorem}

\szcomment{Moved the proof to appendix. }



==> sections/misc_improve.tex <==
\section{Improvement of loss}

Can we improve the dependency on $C$ to $\log\log T$ or $\log C$? 

If interval not marked dishonest, then $O(1)$ regret if the interval was corrupted. 

When an interval has been marked dishonest, algorithm 1 searches from scratch for the current interval, thus it takes $O(\log T)$ rounds for the interval to split. If the interval were corrupted, this leades to $O(C\log T)$ regret. 




Idea 1: When an interval marked dishonest, do not start from scratch. Instead, follow the path up and search. 

Idea 2: Perform Binary search on the path. 

\iffalse
I give some instantiations of the theorem. 
\begin{example}
Let $g(x) = x^{1/u}$ where $u \in (0,1)$. The loss can be bounded as
\begin{align*}
    L\cdot \Tilde{O}(Ng^{-1}(T/N) + g(C) + T\eta ) &\le L\cdot \Tilde{O} (T^u N^{1-u} + C^{1/u} + T\eta) \\
    &\le L \cdot \Tilde{O}\left( T^u (\eta^{-d})^{1-u} + T^u C^{1-u} + C^{1/u} + T\eta \right)
\end{align*}
Choose $\eta = T^{-\frac{1-u}{d(1-u) + 1}}$. Then the total pricing loss is
\[
L \cdot \Tilde{O} (T^{\frac{(1-u)d + u}{(1-u)d + 1}} + T^u C^{1-u} + C^{1/u}). 
\]
\begin{itemize}
\item If $C$ has the order $ C = \Theta(T^{\varepsilon})$ for some $\varepsilon = (0,1)$, the learner can then subsequently choose $u$ to balance the terms. 
\item When the corruption level $C$ is unknown, this work recommend setting $u = \frac{d}{d+1}$, this achieves a regret bound of
\[
L\cdot \tilde{O} \left(   \right)
\]
\szcomment{TODO}
\end{itemize}
\end{example}

\begin{example}
If $C$ can treated as a constant, then the learner can choose $g(x) = 2^x - 1$ and set $\eta = T^{-\frac{1}{d+1}}$. Then the total pricing loss is
\[
L \cdot \Tilde{O} (T^{\frac{d}{d+1}} + \exp(C)). 
\]
\end{example}
\fi
